Percentile Policies for Tracking of Markovian Random Processes with Asymmetric Cost and Observation

Motivated by wide-ranging applications such as video delivery over networks using Multiple Description Codes, congestion control, and inventory management, we study the state-tracking of a Markovian random process with a known transition matrix and a finite ordered state set. The decision-maker must select a state as an action at each time step to minimize the total expected cost. The decision-maker is faced with asymmetries both in cost and observation: in case the selected state is less than the actual state of the Markovian process, an under-utilization cost occurs and only partial observation about the actual state is revealed; otherwise, the decision incurs an over-utilization cost and reveals full information about the actual state. We can formulate this problem as a Partially Observable Markov Decision Process which can be expressed as a dynamic program based on the last full observed state and the time of full observation. This formulation determines the sequence of actions to be taken between any two consecutive full observations of the actual state. However, this DP grows exponentially in the number of states, with little hope for a computationally feasible solution. We present an interesting class of computationally tractable policies with a percentile structure. A generalization of binary search, this class of policies attempt at any given time to reduce the uncertainty by a given percentage. Among all percentile policies, we search for the one with the minimum expected cost. The result of this search is a heuristic policy which we evaluate through numerical simulations. We show that it outperforms the myopic policies and under some conditions performs close to the optimal policies. Furthermore, we derive a lower bound on the cost of the optimal policy which can be computed with low complexity and give a measure for how close our heuristic policy is to the optimal policy.

==> appendices.tex <==
\section{}\label{app:comp}

\begin{proof}[\textbf{Proof of Proposition \ref{prop:compPT}}]
To compute the action sequences and the expected cost of the percentile policy with given thresholds we need to compute $W^{per}_0(s)$ and $W^{per}_0(b_0)$ of percentile policy for all $s\in\mathcal{M}$ and $t=0,...,T-1$. 
The complexity of functions are as follows:
\begin{itemize}
\item $\underline{\pi}^{per}_{s,t}(t')$ for any $t'$ and given $s,t$, $h_{s,t}$ and transitions: $\Theta(M+1)$,
\item To compute $_{\underline{a}}P(s_1,s_2,\tau)$ for all $s_1,s_2,\tau$ and action sequences with the length of $T-t$: $\Theta((T-t)(M+1)^2)$,
\item $\Gamma(s,t)$ for given parameters above: $\Theta((T-t)\times (M+1))$,
\end{itemize}

In total, given $W^{per}_{t'}(s')$ for all $s'$ and $t'=t+1,...,T-1$, to compute $W^{per}_t(s)$ for a given threshold and $s$, we need $\Theta((T-t)(M+1)^2)$ computations. Thus for all $s\in \mathcal{M}$ we need $(M+1)\times \Theta((T-t)(M+1)^2)$ computations.

Now to compute all action sequences and expected costs, we use backward recursion on time from horizon $T-1$ to $0$.
 Thus, for $t=T-1$ the complexity is simply $\Theta(M+1)$. We use the already computed values at time $t+1,...,T-1$ to compute the minimum cost and the action sequences at time $t$. 
Thus, the total complexity of percentile policy equals to $\Theta(\sum_{t=0}^{T-1} (T-t)\times(M+1)^3)=\Theta(T^2 (M+1)^3)$.
\end{proof}


\section{}\label{app_lproofs}

\begin{proof}[\textbf{Proof of Proposition \ref{C_mybb1}}]
The proof is straightforward using the uni-modality of expected immediate cost given in the following lemma.
\begin{lem} \label{Myopic_cor}
The expected immediate cost for any belief $b$ is a uni-modal function of the action $r$, where a function is called uni-modal iff it has at most one minimum and being decreasing/increasing before/after the minimum.
\end{lem}

Thus the expected immediate cost is decreasing with respect to $r$ when $\sum_{i=m}^{r} {b(i)} < \frac{c_l}{c_l+c_u}$ and it is increasing otherwise. Therefore, the myopic action which minimizes the expected immediate cost, given in (\ref{eq:myopic}), is equal to the lowest action $r$ satisfying the inequality $\sum_{i=m}^{r} {b(i)} \geq \frac{c_l}{c_l+c_u}$.
\end{proof}
%\medskip

\begin{proof}[\textbf{Proof of Lemma \ref{Myopic_cor}}]
To prove this lemma, let us compute the derivative of the expected immediate cost for the belief vector $b$ with respect to action $r$ given in (\ref{eq:vfnR}),
\begin{align}
\Delta \bar C(b;r)&=\bar C(b;r+1)-\bar C(b;r) =(c_l+c_u) \sum_{i=m}^{r} {b(i)}-c_l.\nonumber% \label{eq:c2}
\end{align}
It's easily seen that if the inequality in (\ref{eq:rmc1}) holds, $\Delta \bar C(b;r)\geq 0$. Otherwise it is negative. This concludes that $\bar C(b;r)$ is uni-modal with unique minimum at the myopic action given in (\ref{eq:rmc1}).
\end{proof}
%\medskip


\section{}\label{sec:special}

\textbf{Optimal Policy for Special Cases:}
Even though computing the optimal policy is intractable in general, there are some trivial cases in which the optimal policy is achievable. In the following subsections, we present simple special cases of zero under/over utilization costs, %static/drift processes (special $P$ matrices), 
and cases where the myopic policy is optimal. 


\subsection{\textbf{Zero Under-utilization or Over-utilization Cost}}

For two special cases the optimal policy is trivial. First if the under-utilization cost coefficient is zero, $c_l=0$, the optimal policy selects the lowest actions $0$ all the time or any action sequences in which the transition probabilities to the actions below them are zero, \textit{i.e.}, for any full observation of state $s$ at time $t$, $\underline{\pi}^{opt}_{s,t}(\tau) \leq \min \{i: P^{\tau-t}_{s,i}\neq 0\}$ for $\tau=t+1,...T$, $s\in\mathcal{M}$.
Second, if the over-utilization cost coefficient is zero, $c_u=0$, the optimal policy selects the highest action $1$ all the time or any action sequences in which the transition probabilities to the actions above them are zero, \textit{i.e.}, $\underline{\pi}^{opt}_{s,t}(\tau) \geq \max \{i: P^{\tau-t}_{s,i}\neq 0\}$ for $\tau=t+1,...T$, $s\in\mathcal{M}$. 
Note that the total expected (discounted) costs achieved by the optimal policy for these two trivial cases are always zero. 
The optimal policy for zero under/over-utilization cost is also a percentile policy with a threshold of zero/one. 


\subsection{\textbf{Cases where Myopic Policy is Optimal}}
There are some cases where the optimal policy is equivalent to the myopic policy, given by:
\begin{itemize}
\item Zero discount factor ($\beta=0$),
\item Independent and Identically Distributed (i.i.d.) Processes,
\item When there is no ambiguity about the future, \textit{i.e.} the rows of the transition matrix are equal to a fixed unit vector. $P_{i,.}=I_{a}, \forall i\in \mathcal{M}$ for a given $a\in \mathcal{M}$ where $I_a$ is a $M+1$-dimensional unit vector with 1 in the $a$-th position and zero elsewhere.
\end{itemize}

Thus the myopic policy is a percentile policy with the threshold of $h^{m}=\frac{c_l}{c_l+c_u}$. 



\subsection{\textbf{Any transition matrix with unit vectors as rows}}
Here we consider the cases where each row of the matrix is a unit vector, \textit{i.e.} there is only one 1 in any row and the rest of the elements are zero, \textit{e.g.} a static process with matrix $P=I$. For these cases, after any full observation
of state $s\in \mathcal{M}$ at time $t=0,...,T-1$, the actual state is simply known for the rest of the times with probability one. Therefore the optimal policy selects the actions equal to the actual states $\underline{\pi}^{opt}_{s,t}(\tau)=\{i: P^{\tau-t}(i)=1\}$ for $\tau=t+1,...,T$ and the expected cost-to-go is zero. 



\section{}\label{app_beliefDP}

We could alternatively represent the decision problem based on the decision-maker's belief, \textit{i.e.} his posterior probability on the hidden state $B_t$ at each time step conditioned on past actions and observations (\cite{mansourifard2013bayesian, mansourifard2015, bensoussan2007multiperiod}).
Let the conditioned probability distribution of the state, given all past observations, is denoted by a belief vector $b_t=[b_t(0),...,b_t(M)]$, with elements of $b_t(k)=Pr(B_t=k|~past~observations), k \in \mathcal{M}$. In other words, $b_t$ represents the probability distribution of $B_t$ over all possible states in $\mathcal{M}$.
In this representation, the goal is to make a decision at each time step based on the history of observations; but due to the lack of full information, the decision-maker may only make the decision based on the belief vector. 
It can be shown that the belief vector is a sufficient statistic of the complete observation history (see \textit{e.g.}, \cite{smallwood1973optimal}). Note that to find the optimal action at each time, we need to know the history of actions and observations. The belief vector is a function of these parameters and is updated every time step based on the selected action and the observation, since all the actions and observations could effect the probability distribution of the states. Thus, all the history is compressed in the belief vector.

Here, we present the belief-based DP which results in the same optimal policy as the sequence-based DP presented in the main text,
as the following recursive equations: 
\begin{subequations}
\begin{align}
&V_t(b_t):=\min_{r_t} V_t(b_t;r_t), \label{eq:vfnmin}\\
&V_T(b_T;r_T)=\bar C_{T}(b_T;r_T),\label{eq:vfnT}\\
&V_t(b_t;r_t):=\bar C(b_t;r_t)+\beta \mathbb{E}\{V_{t+1}(b_{t+1})|r_t,b_t\},\ \ t<T  \label{eq:vfn}
\end{align}
\end{subequations}
where $b_{t+1}$ is the updated belief vector. It can be computed given the action $r_t$ and observations.
The value function $V_t(b_t)$  is the minimum expected cost-to-go when the current belief vector is $b_t$. 
Note that $V_t(b_t;r)$ is the expected cost-to-go after time $t$ under belief $b_t$ and action $r$ at time $t$ and following the optimal policy for time $t+1$ onward, with updated belief vector according to the action $r$.

The belief updating maps current belief vector, selected action, and the observation to the belief vector for the next time step:
\begin{align}\label{eq:pt1}
b_{t+1} = \begin{cases}
  T_{r_t}[b_{t}] P  &\text{if}\ B_t\geq r_t, \\
 I_{i}P  &\text{if}\  B_t=i<r_t,\\
\end{cases}\
\end{align}
where $I_{i}$ is the $M+1$-dimensional unit vector with 1 in the $i$-th position and 0 otherwise. Note that $I_{i}P$ is equivalent to the $i$-th row of matrix P, \textit{i.e.} $P_{i,.}$.
$T_{r}$ is a non-linear operation on a belief vector $b$, as follows:
\begin{align}\label{eq:Trp}
T_{r}[b](i) = \begin{cases}
  0  &\text{if}\ i < r, \\
 \frac{b(i)}{\sum_{j=r}^M b(j)}  &\text{if}\  i\geq r.\\
\end{cases}\
\end{align}
The update of the belief vector is derived in two steps. First step: when we get full observation about the actual state $i$ with taking action $r_t$, \textit{i.e.} when $i<r_t$, the probability distribution of the state could be updated to $I_i$, since we are sure that the probability of actual state being different than $i$ is zero.
And when we get partial observation that the actual state is higher than $r_t$, we can update the probability distribution as follows: force the probability of the actual state being less than $r_t$ to be zero and normalize the rest of the probabilities to sum up to one. Second step: the above updating corresponds to the probability distribution at the same time step of taking action and observation. But we need a new probability distribution (belief vector) for the next time step. Thus we multiply the updated distribution with transition matrix $P$.

The future expected (discounted) cost can be computed as follows:
\begin{align}
\mathbb{E}\{V_{t+1}(b_{t+1})|r_t,b_t\}&=\sum_{i=r_t}^M {b_t(i)} V_{t+1}(T_{r_t}[b_{t}]P)\nonumber\\
&+\sum_{i=0}^{r_t-1} {b_t(i)V_{t+1}(P_{i,.})}.\label{eq:vfnR3}
\end{align}
Note that for all $t=1,...,T$, $V_t(b_t)=\min_{\pi} J^{\pi}_{T-t}(b_t)$ with probability 1. In particular, $V_1(b_1)=J_T^{\pi}(b_1)$.
A policy $\pi^{opt}$ is optimal if for $t=1,...,T$; $r_t^{opt}(b_t)$ achieves the minimum in (\ref{eq:vfnmin}), denoted by: %%% =\pi^{opt}
\begin{align}%\label{eq:optimalv}
r_t^{opt}(b_t):=\arg\min_{r \in \mathcal{M}} V_t(b_t;r).\nonumber
\end{align}

This DP is equivalent to the DP given in Section \ref{sec:seqDP} as follows:
\begin{align}
&V_t(P_{i,.})=W_{t-1}(i), \nonumber\\
&V_0(b_0)=W(b_0),\nonumber\\
&r_{\tau}^{opt}(b_{\tau})=\underline{\pi}^{opt}_{s^{FO},t^{FO}}(\tau),\nonumber
\end{align}
where $b_{\tau}$ is the updated belief using (\ref{eq:pt1}) based on the optimal actions at times $t+1,...,\tau-1$ (propagated from $b_{t}=I_s$) and $t^{FO}$ is the last time of full observation to the state $s^{FO}$ before $\tau$.


\section{}\label{app:PBFO}

To prove Proposition \ref{prop:FO}, we use the belief-based DP presented in Appendix \ref{app_beliefDP} and it is enough to prove the following lemma:

\begin{lem}\label{prop:FO2}
The cost-to-go of the optimal policy is lower bounded by the cost-to-go of the full observation (FO) case under the same belief vector, \textit{i.e.},
\begin{align}\label{eq:FO2}
V_t(b_t) \geq V^{FO}_t(b_t).
\end{align}
\end{lem}

We need the following lemma about the concavity of cost-to-go functions to prove Lemma \ref{prop:FO2}.

\begin{lem}\label{L_convvf}
The expected discounted cost-to-go accrued under action $r$, $V_t(b;r)$, and the value function, $V_t(b)$, are concave with respect to the belief vector $b$,
\textit{i.e.}
\begin{align}\label{eq:convf}
&V_t(b;r)\geq \lambda V_t(b_1;r)+(1-\lambda)V_t(b_2;r),\ \ \forall r\in \mathcal{M}, \nonumber\\
&V_t(b)\geq \lambda V_t(b_1)+(1-\lambda)V_t(b_2),\ \ \forall 0\leq \lambda \leq 1.
\end{align}
\end{lem}


\begin{proof}[\textbf{Proof of Lemma \ref{L_convvf}}]
We use induction to prove the concavity of $V_t(b;r)$ with respect to the belief vector, $b$, for finite horizon.
Let's assume $b$ is a linear combination of two belief vectors $b_1$ and $b_2$, such that:
\begin{align}\nonumber%\label{eq:b}
b=\lambda b_1+(1-\lambda) b_2, 0\leq \lambda \leq 1.
\end{align}

At horizon $T$, the immediate cost, as given in (\ref{eq:vfnR}), is affine linear with respect to the belief vector. In other words,
\begin{align}\label{eq:affT}
\bar C(b;r)&=\lambda \bar C(b_1;r)+ (1-\lambda) \bar C(b_2;r).\end{align}
which confirms the concavity of the expected cost-to-go at horizon $T$.
Now assuming $V_{t+1}(.)$ is concave, we will consider $V_t(.)$. Using (\ref{eq:vfn}) and (\ref{eq:vfnR3}) we have:

\begin{align}
V_t(&b;r)-\lambda V_t(b_1;r) -(1-\lambda) V_t(b_2;r) \nonumber\\
&=[C(b;r)-\lambda \bar C(b_1;r)\nonumber\\
&- (1-\lambda) \bar C(b_2;r)] -(1-\lambda) V_{t+1}(T_r [b_2] P)\sum_{i=r}^{M} {b_2(i)})\nonumber\\ %\label{eq:conv12}\\
&+\beta(V_{t+1}(T_r [b] P)\sum_{i=r}^{M} {b(i)}-\lambda V_{t+1}(T_r [b_1] P)\sum_{i=r}^{M} {b_1(i)},\nonumber\\
\end{align}
and from (\ref{eq:affT}) and  $\lambda'=\lambda \frac{\sum_{i=r}^{M} {b_1(i)}}{\sum_{i=r}^{M} {b(i)}}$:
\begin{align}
V_t(b;r)&-\lambda V_t(b_1;r) -(1-\lambda) V_t(b_2;r) \nonumber\\
&=\beta \sum_{i=r}^{M} {b(i)} [V_{t+1}(T_r [b] P)-\lambda' V_{t+1}(T_r [b_1] P)\nonumber\\
&-(1-\lambda') V_{t+1}(T_r [b_2] P)], \nonumber% \label{eq:convl}
\end{align}


Let $j\geq r$:
\begin{align}%\label{eq:lamp}
&\lambda' T_r [b_1](j)+(1-\lambda') T_r [b_2](j)\nonumber\\
&=\frac{\lambda \sum_{i=r}^{M} {b_1(i)} T_r [b_1](j) + (1-\lambda)\sum_{i=r}^{M} {b_2(i)} T_r [b_2](j)}{\sum_{i=r}^{M} {b(i)}} \nonumber\\
&=\frac{1}{\sum_{i=r}^{M} {b(i)}}[\lambda \sum_{i=r}^{M} {b_1(i)} \frac{b_1(j)}{\sum_{i=r}^{M} {b_1(i)}} \nonumber\\
&+ (1-\lambda)\sum_{i=r}^{M} {b_2(i)} \frac{b_2(j)}{\sum_{i=r}^{M} {b_2(i)}}]
  \nonumber\\
&=\frac{\lambda b_1(j) + (1-\lambda)b_2(j)}{\sum_{i=r}^{M} {b(i)}}=\frac{b(j)}{\sum_{i=r}^{M} {b(i)}}=T_r [b](j),\nonumber
\end{align}
and for $j<r$, $T_r [b_1](j)+(1-\lambda') T_r [b_2](j)=0$.
Multiplying by $P$, we have $\lambda' T_r [b_1]P+(1-\lambda') T_r[b_2]P=T_r[b]P$. The induction step follows the concavity of $V_{t+1}(.)$.

To prove the concavity of value function, $V_t(b)$, with respect to $b$ we use the definition of (\ref{eq:vfnmin}) to get:
\begin{subequations}
\begin{align}
&V_t(b)=\min_{r}{V_t(b;r)}=V_t(b;r^*) \label{eq:pfl2}\\
&\geq \lambda V_t(b_1;r^*)+(1-\lambda)V_t(b_2;r^*)\label{eq:pfl21}\\
&\geq \lambda \min_{r_1}{V_t(b_1;r_1)}+(1-\lambda)\min_{r_2}{V_t(b_2;r_2)}\label{eq:pfl22}\\
&=\lambda V_t(b_1)+(1-\lambda)V_t(b_2),\label{eq:pfl23}
\end{align}
\end{subequations}
where $r^*=\arg \min_{r}{V_t(b;r)} $ and (\ref{eq:pfl21}) is the result of the lemma for $V_t(b;r^*)$ and applying the definition of (\ref{eq:vfnmin}) one more time in (\ref{eq:pfl23}) completes the proof.
\end{proof}
%\medskip


\begin{proof}[\textbf{Proof of Lemma \ref{prop:FO2}}]
First, the cost-to-go function of FO policy can be computed as:
\begin{align}
V^{FO}_t(b_t,r)=\bar C(b_t; r)+\beta \sum_{i=0}^{M} b_t(i) V^{FO}_{t+1}(P_{y,.}),\nonumber
\end{align}
Thus the optimal policy for FO policy is equivalent to the myopic policy since the second term is independent of the action $r$ and,
\begin{align}
\arg \min_r V^{FO}_t(b_t,r)=\arg \min_r \bar C(b_t; r).\nonumber
\end{align}
Therefore,
\begin{align}\nonumber
V^{FO}_t(b_t)=\bar C(b_t; \pi^{myopic}(b_t))+\beta \sum_{i=0}^{M} b_t(i) V^{FO}_{t+1}(P_{i,.}).
\end{align}
Now to prove the proposition we use induction. Fist, at $t=T$ we have:
\begin{align}
V_T(b_T)&- V^{FO}_T(b_T)\nonumber\\
&=\min_r \bar C(b_T; r)-\bar C(b_T; \pi^{myopic}(b_T))= 0,\nonumber
\end{align}
since the optimal action and the myopic action are equivalent at the horizon.
Now assuming (\ref{eq:FO}) is true at time steps $t+1$ onwards, we should prove it for time $t$.
\begin{align}
V_t(b_t)-& V^{FO}_t(b_t)=\bar C(b_t; r^{opt}(b_t))\nonumber\\
&+\beta \sum_{i=0}^{r^{opt}(b_t)-1}b_t(i) V_{t+1} (P_{i,.})\nonumber\\
&+\beta \sum_{i=r^{opt}(b_t)}^M b_t(i) V_{t+1} (T_{r^{opt}(b_t)}[b_{t}]P)\nonumber\\
&-\bar C(b_t; \pi^{myopic}(b_t))-\beta \sum_{i=0}^{M} b_t(i) V^{FO}_{t+1}(P_{i,.}), \nonumber
\end{align}
where $T_{r^{opt}(b_t)}[b_{t}]P=\frac{\sum_{j=r^{opt}(b_t)}^M b_t(j)P_{j,.}}{\sum_{i=r^{opt}(b_t)}^M b_t(i)}$.
We use the concavity of the value function to get the following inequality:
\begin{align}\label{eq:conc}
V_{t+1} (T_{r^{opt}(b_t)}[b_{t}]P) \geq
\frac{\sum_{i=r^{opt}(b_t)}^M b_t(i)V_{t+1} (P_{i,.})}{\sum_{j=r^{opt}(b_t)}^M b_t(j)}.
\end{align}
Therefore, by applying (\ref{eq:conc}) and merging two summations:
\begin{subequations}
\begin{align}
V_t(b_t)-& V^{FO}_t(b_t)\nonumber\\
&=[\bar C(b_T; r^{opt}(b_t))-\bar C(b_T; \pi^{myopic}(b_T))]\label{eq:FOind2-a}\\
&+\beta \sum_{i=0}^{M}b_t(i) [V_{t+1} (P_{i,.})-V^{FO}_{t+1}(P_{i,.})]\geq 0. \label{eq:FOind2-b}
\end{align}
\end{subequations}
The term in (\ref{eq:FOind2-a}) is greater than or equal to zero based on the definition of the myopic policy. The term in (\ref{eq:FOind2-b}) is also greater than or equal to zero using the induction assumption at $t+1$. Thus the whole expression is greater than or equal to zero and the proof is complete.
\end{proof}


